Machine Translation Evaluation with Neural Networks

We present a framework for machine translation evaluation using neural networks in a pairwise setting, where the goal is to select the better translation from a pair of hypotheses, given the reference translation. In this framework, lexical, syntactic and semantic information from the reference and the two hypotheses is embedded into compact distributed vector representations, and fed into a multi-layer neural network that models nonlinear interactions between each of the hypotheses and the reference, as well as between the two hypotheses. We experiment with the benchmark datasets from the WMT Metrics shared task, on which we obtain the best results published so far, with the basic network configuration. We also perform a series of experiments to analyze and understand the contribution of the different components of the network. We evaluate variants and extensions, including fine-tuning of the semantic embeddings, and sentence-based representations modeled with convolutional and recurrent neural networks. In summary, the proposed framework is flexible and generalizable, allows for efficient learning and scoring, and provides an MT evaluation metric that correlates with human judgments, and is on par with the state of the art.

==> discussion-new-shafiq.tex <==
%!TEX root = neural-mte-csl.tex
%-------------------------------------------------------
% Machine Translation Evaluation with Neural Networks
% Paper submitted to Computer Speech and Language
% April 2016
%-------------------------------------------------------
% Section 6: Discussion - NEW topics: Shafiq
%-------------------------------------------------------

\subsection{Sentence-based representation of input texts}
\label{subsec:lstms}

\noindent One aspect in which our proposed model is extremely simple is that it computes the semantic representation of a sentence by just \emph{averaging} the embedding vectors of its words. In this bag-of-words (BOW) approach, we disregard the structure (e.g., word order) and the compositionality of phrases in a sentence. In this section, we explore Recurrent Neural Networks (RNN) with a Long Short Term Memory (LSTM) hidden layer~\cite{hochreiter1997long} to perform semantic composition of phrases and fine-tuning of word vectors simultaneously.
%\footnote{we could have used CNNs...} 

As shown in Figure~\ref{fig:lstm-framework}a, RNNs encode a sentence into a vector by processing its words sequentially, at each time step combining the current input with the previous hidden state. We experiment with both unidirectional and bidirectional RNNs.    



\begin{figure*}[tb!]
\scalebox{0.98}{
\begin{subfigure}{.60\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{imgs/lstm-rnn}
  \caption{Bidirectional LSTM for sentence representation}
  \label{fig:sfig1}
\end{subfigure}
\begin{subfigure}{.40\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{imgs/lstm-cell}
  \caption{An LSTM cell}
  \label{fig:sfig2}
\end{subfigure}}
\caption{LSTM-based recurrent neural network for sentence representation}
\label{fig:lstm-framework}
\end{figure*}

%Given an input sentence $\mathbf{s} = (w_1, \cdots, w_T)$, we first transform it into a feature sequence by mapping each token $w_t \in \mathbf{s}$ to an index in $E$, and generate an input vector $\mathbf{x_t}\in\real^{D}$ for each token $w_t$.

In this setting, we first map each token $w_t$ to an embedding vector  $\mathbf{x_t}$. %$\in\real^{D}$ by multiplying the corresponding one-hot vector by the embedding matrix. 
The input vectors are then passed to the LSTM recurrent layer, which computes a compositional representation $\overrightarrow{\mathbf{h}}_t$ at every time step $t$ by performing nonlinear transformations of the current input  $\mathbf{x}_t$ and the output of the previous time step $\overrightarrow{\mathbf{h}}_{t-1}$. Specifically, the recurrent layer in an LSTM RNN is formed by hidden units called \emph{memory blocks}. A memory block is composed of four elements: \Ni a memory cell $c$ (a neuron) with a self-connection, \Nii an input gate $i$ to control the flow of input signal into the neuron, \Niii an output gate $o$ to control the effect of the neuron activation on other neurons, and \Niv a forget gate $f$ to allow the neuron to adaptively reset its current state through the self-connection. The following sequence of equations describe how the memory blocks are updated at every time step $t$: 

\begin{eqnarray}
	\mathbf{i}_t &=& \sig(U_i\mathbf{h}_{t-1} + V_i\mathbf{x}_t + \mathbf{b}_i)  \label {lstm_first}\\
    \mathbf{f}_t &=& \sig(U_f\mathbf{h}_{t-1} + V_f\mathbf{x}_t + \mathbf{b}_f) \\
    \mathbf{c}_t &=& \hspace{-0.1cm}  \mathbf{i}_t\odot \tanh(U_c\mathbf{h}_{t-1} + V_c\mathbf{x}_t) + \mathbf{f}_t\odot\mathbf{c}_{t-1} \\
    \mathbf{o}_t &=& \sig(U_o\mathbf{h}_{t-1} + V_o\mathbf{x}_t + \mathbf{b}_o) \\
    \mathbf{h}_t &=& \mathbf{o}_t \odot \tanh(\mathbf{c}_t) \label {lstm_last}
%    y_t &=& W_{hy}h_t + b_y
\end{eqnarray}

\noindent where $U_k$ and $V_k$ are the weight matrices between two consecutive hidden layers, and between the input and the hidden layers, respectively, which are associated with gate $k\in$ \{input, output, forget, cell\}; and $\mathbf{b}_k$ is the corresponding bias vector. The symbols $\sig$ and $\tanh$ denote hard sigmoid and hyperbolic tangent, respectively, and the symbol $\odot$ denotes an element-wise product of two vectors.
 
LSTM, by means of its specifically designed gates (as opposed to simple RNNs), is capable of capturing long range dependencies. We can interpret $\mathbf{h}_t$ as an intermediate representation summarizing the past. The output of the last time step $\overrightarrow{\mathbf{h}_T}$ thus represents the whole sentence, which can be fed to the subsequent layers of the neural network architecture. 

\paragraph{Bidirectionality} 
The RNN described above encodes information from the past only. However, information from the future could also be crucial, especially for longer sentences, where a unidirectional RNN can be limited in encoding the necessary information into a single vector. Bidirectional RNNs \cite{Schuster:1997} capture dependencies from both directions, thus providing two different views of the same sentence. This amounts to having a backward counterpart for each of the equations from \ref{lstm_first} to \ref{lstm_last}. Each sentence in a bidirectional LSTM RNN is thus represented by the concatenated vector $[\overrightarrow{\mathbf{h}_T},\overleftarrow{\mathbf{h}_T}]$, where $\overrightarrow{\mathbf{h}_T}$ and $\overleftarrow{\mathbf{h}_T}$ are the encoded vectors summarizing the past and the future, respectively.

\paragraph{Results} 
In our experiments, we use the neural architecture shown in Figure \ref{fig:architecture} with one notable difference: we exclude the averaged semantic vectors (\wiki), and instead we use the LSTM RNN (Figure~\ref{fig:sfig1}) to encode the vectors for the sentences. Complex neural models like LSTMs tend to overfit because of the increased number of parameters. To avoid overfitting, we use dropout \cite{hinton:dropout} of embedding and hidden units and perform early stopping based on the accuracy on the development set. We experimented with the following dropout rates: $0.0, 0.25, 0.5, 0.75$. To compare to the best baseline results, we initialize $E$ with the pretrained \wiki\ word vectors \cite{pennington-socher-manning:2014:EMNLP2014}, and we do fine-tuning of these vectors. The number of units in the LSTM layer was fixed to $50$.  

\begin{table*}[t]
\centering
%\vspace{-2mm}
%\hspace*{-8mm}
{\footnotesize\begin{tabular}{lccccc}
\toprule
   & \multicolumn{5}{c}{\bf Kendall's $\tau$} \\\cmidrule(l{2pt}r{2pt}){2-6}
\multicolumn{1}{c}{\bf Details} & { \bf cz }&{\bf de} & {\bf es}  & {\bf fr} &{\bf AVG}\\
\midrule
Averaging (no LSTM) & 26.92  & 33.05 &  29.83 &  29.01&  29.70\\
\midrule
Unidirectional LSTM  & 25.51 & 33.31 & 30.40 & 29.16 & 29.59\\
Bidirectional LSTM   & 26.20 & 33.82 & 30.16 & 29.23 & \textbf{29.85} \\
Bidirectional LSTM  (random) & 25.91 & 33.81 & 30.44 & 28.90 &  29.76 \\
%Bidirectional LSTM - syntax  & 26.31 & 32.30 & 29.31 & 29.20 &  29.28 \\
%Bidirectional LSTM + tensor &&  &  &  &  \\
\bottomrule
\end{tabular}}
\caption{\label{tab:lstm-discussion}{\small Kendall's $\tau$ on WMT12 for different variants of LSTM RNNs. }}
\end{table*}

Table \ref{tab:lstm-discussion} shows the results on the WMT12 testset for different variants of LSTM RNNs. The first row shows the results for the averaging baseline (no semantic composition using LSTM). The second row shows the results of our model with a unidirectional LSTM. We can notice that even though the unidirectional LSTM outperforms the baseline in three out of four languages, it fails to beat the baseline on average because of its poor performance on Czech. 
%
%The third row shows the results of our model with a bidirectional LSTM. 
Bidirectional LSTM (third row) yields an average improvement of $+0.15$ over the baseline. Finally, the fourth row shows the results of the model when word vectors are randomly initialized (as oppposed to pretrained). %in the bidirectional LSTM. 
This model performs slightly better than the baseline on average, which means that bidirectional LSTMs can achieve good results even without pretrained word vectors. 

We notice that our models with LSTM-based semantic composition fail to achieve better results for Czech. This could be due to the reordering errors made by Czech-English traslation systems, for which sequential LSTMs  may not be robust enough to encode the necessary information. %to distinguish two candidate translations. 

Another general observation is that fine tuning and composition with LSTMs did not yield improvements to the extent that we had expected. One potential reason could be that the compositional aspect is partially captured by the syntactic embeddings, which are produced as the parser composes phrases hierarchically using a recursive neural network \cite{socher-EtAl:2013:ACL2013}. To investigate this, %hypothesis, 
Table~\ref{tab:lstm-discussion2} shows the results of the baseline and the model with LSTM after excluding the syntactic embeddings. In this setting, LSTM yields a larger gain of $+0.31$.

%the last row of  We see that the results drop by only $-.57$.    

\begin{table*}[t]
\centering
%\vspace{-2mm}
%\hspace*{-8mm}
{\footnotesize\begin{tabular}{lccccc}
\toprule
   & \multicolumn{5}{c}{\bf Kendall's $\tau$} \\\cmidrule(l{2pt}r{2pt}){2-6}
\multicolumn{1}{c}{\bf Details} & { \bf cz }&{\bf de} & {\bf es}  & {\bf fr} &{\bf AVG}\\
\midrule
%Averaging baseline -syntax & 26.92  & 33.05 &  29.83 &  29.01&  29.70\\
Averaging baseline $-$ syntax & 25.67 & 32.50 & 29.21 & {28.92} & 29.07 \\
%\midrule
Bidirectional LSTM $-$ syntax  & 26.31 & 32.60 & 29.31 & 29.20 &  29.38 \\
\bottomrule
\end{tabular}}
\caption{\label{tab:lstm-discussion2}{\small Results for baseline and LSTM-based model without syntactic embeddings. }}
\end{table*}


==> setup.tex <==
%!TEX root = neural-mte-csl.tex
%-------------------------------------------------------
% Machine Translation Evaluation with Neural Networks
% Paper submitted to Computer Speech and Language
% April 2016
%-------------------------------------------------------
% Section 4: Experimental setup
%-------------------------------------------------------

%\begin{itemize}
%\item Subsection 1: WMT corpora description and task evaluation measures
%\item Subsection 2: Explain the training setting for the NN model: early stopping, parameters and parameter tuning, pre-training, etc.
%\end{itemize}

In this section, we describe the different aspects of our general experimental setup (we will discuss some extensions thereof in Section~\ref{sec:discussion}), starting with a description of the input representations we use to capture the syntactic and semantic characteristics of the two hypothesis translations and the corresponding reference, as well as the datasets used to evaluate the performance of our model.

\subsection{Word Embedding Vectors}

Word embeddings play a crucial role in our model, since they allow us to model complex relations between the translations and the reference using syntactic and semantic vector representations. \\
 %In our experiments, we experiment with syntactic and semantic vectors as a representation for a sentence.

\vspace{-2mm}
\noindent{\bf Syntactic vectors}. 
We generate a syntactic vector for each sentence\
using the Stanford neural parser \cite{socher-EtAl:2013:ACL2013},
which generates a 25-dimensional vector as a by-product of syntactic parsing using a recursive NN.
Below we will refer to these vectors as \syntax.\\

\vspace{-2mm}
\noindent{\bf Semantic vectors}. 
We compose a semantic vector for a given sentence
using the average of the embedding vectors for the words it contains~\cite{Mitchell:Lapata:2010}.
We use pre-trained, fixed-length word embedding vectors produced by 
\Ni GloVe \cite{pennington-socher-manning:2014:EMNLP2014},
\Nii COMPOSES \cite{P14-1023},
and
\Niii word2vec \cite{mikolov-yih-zweig:2013:NAACL-HLT}.

Our primary representation is based on 50-dimensional GloVe vectors,
trained on Wikipedia 2014+Gigaword 5 (6B tokens),
to which below we will refer as \wiki. 

Furthermore, we experiment with \wikii, the 300-dimensional GloVe vectors trained on the same data,
as well as with the \commoncrawl \ and \commoncrawll,
300-dimensional GloVe vectors trained on 42B and on 840B tokens from Common Crawl.

We also experiment with the pre-trained, 300-dimensional word2vec embedding vectors, or \wordvec,
trained on 100B words from Google News.
Finally, we use \composes, the 400-dimensional COMPOSES vectors trained on 2.8 billion tokens
from ukWaC, the English Wikipedia, and the British National Corpus.




\subsection{Tuning and Evaluation Datasets}

We experiment with datasets of segment-level human rankings of system outputs
from the WMT11, WMT12 and WMT13 Metrics shared tasks \cite{WMT11,WMT12,WMT13}.
We focus on translating into English,
for which the WMT11 and WMT12 datasets can be split by source language:
Czech (cz), German (de), Spanish (es), and French (fr);
WMT13 also has Russian (ru).
%There were about 10,000 non-tied human judgments per language pair per dataset.


\subsection{Evaluation Score}

We evaluate our metrics in terms of correlation with human judgments measured using Kendall's $\tau$.
We report $\tau$ for the individual languages as well as macro-averaged across all languages.

Note that there were different versions of $\tau$ at WMT over the years.
Prior to 2013, WMT used a strict version, which was later relaxed at WMT13 and further revised at WMT14.
See \cite{machacek-bojar:2014:W14-33} for a discussion.
Here we use the strict version used at WMT11 and WMT12.


\subsection{Experimental Settings}

{\bf Datasets}: We train our neural models on WMT11 and we evaluate them on WMT12. 
We further use a random subset of 5,000 examples from WMT13 as a validation set to implement early stopping.

\noindent {\bf Early stopping}: We train on WMT11 for up to 10,000 epochs, and we calculate Kendall's $\tau$ on the development set after each epoch.
We then select the model that achieves the highest $\tau$ on the validation set; in case of ties for the best $\tau$, we select the latest epoch that achieved the highest $\tau$. 

\noindent{\bf Network parameters}: We train our neural network using SGD with adagrad, an initial learning rate of $\eta=0.01$, mini-batches of size $30$, and $L_2$ regularization with a decay parameter $\lambda =1e^{-4}$. We initialize the weights for our matrices by sampling from a uniform distribution following \cite{Xavier10}. We further set the size of each of our pairwise hidden layers $H$ to four nodes, and we normalize the input data using min-max to map the feature values to the range $[-1,1]$.


